When Like Destabilizes Like: Inverted Solvent Effects in Apolar Nanoparticle Dispersions

We report on the colloidal stability of nanoparticles with alkanethiol shells in apolar solvents. Small angle X-ray scattering and molecular dynamics simulations were used to characterize the interaction between nanoparticles in linear alkane solvents ranging from hexane to hexadecane, including \SI{4}{\nano\meter} gold cores with hexadecanethiol shells and \SI{6}{\nano\meter} cadmium selenide cores with octadecanethiol shells. We find that the agglomeration is enthalpically driven and that, contrary to what one would expect from classical colloid theory, the temperature at which the particles agglomerate increases with increasing solvent chain length. We demonstrate that the inverted trend correlates with the temperatures at which the ligands order in the different solvents, and show that the inversion is due to a combination of enthalpic and entropic effects that enhance the stability of the ordered ligand state as the solvent length increases. We also explain why cyclohexane is a better solvent than hexane, despite having very similar solvation parameters to hexadecane.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
